Mean Opinion Score as a New Metric for User-Evaluation of XAI Methods

This paper investigates the use of Mean Opinion Score (MOS), a common image quality metric, as a user-centric evaluation metric for XAI post-hoc explainers. To measure the MOS, a user experiment is proposed, which has been conducted with explanation maps of intentionally distorted images. Three methods from the family of feature attribution methods - Gradient-weighted Class Activation Mapping (Grad-CAM), Multi-Layered Feature Explanation Method (MLFEM), and Feature Explanation Method (FEM) - are compared with this metric. Additionally, the correlation of this new user-centric metric with automatic metrics is studied via Spearman's rank correlation coefficient. MOS of MLFEM shows the highest correlation with automatic metrics of Insertion Area Under Curve (IAUC) and Deletion Area Under Curve (DAUC). However, the overall correlations are limited, which highlights the lack of consensus between automatic and user-centric metrics.

==> contents/2-acknowledgements.tex <==
\subsubsection{Acknowledgements}
% I would like to thank my supervisor Prof. Jenny Benois-Pineau for her scientific guidance of my internship and her availability for all my questions. I would also like to thank the PhD student A. Zhukov for his patience in the explanations of the psycho-visual experiment Software installation and functioning and to all PhD students and interns from AIV/TAD/I\&S. I am very much grateful to all 31 participants of our experiment from all over the world and I would like to thank Romain Bourqui and LaBRI system engineers for organizing material basis for our psycho-visual experiments. I also thank LaBRI for the financial support of my internship and the IPCV team for the great training program and support. Last but not least, I thank my family for their support. 
% \clearpage

==> contents/6-results-SA-new.tex <==
\section{Results and discussion } \label{sec:result-SA}
% The Code of Studies and Exams recommends the following content for this chapter: "Evaluation, critical analysis of the implemented technical solutions, possibilities for further development."
% However, you are free to structure the content of your thesis as you want
This section presents the results of the statistical analysis of MOS conducted to evaluate the performance of the explanation methods (Grad-CAM \cite{DBLP:journals/corr/SelvarajuDVCPB16}, MLFEM \cite{bourroux:hal-03689004}, and FEM \cite{ahmedasiffuad:hal-02963298}) described in Section \ref{sec:SA}. Then we present and discuss results of the study of positioning of our new user-involvement metric with regard to automatic metrics IAUC and DAUC. 

% The analysis focused on Mean Opinion Score (MOS) as the primary user experience metric. Using the Kruskal-Wallis H test \cite{doi:10.1080/01621459.1952.10483441} and post-hoc Mann-Whitney U test \cite{10.1214/aoms/1177730491}, we investigated potential differences in user perception of the explanation methods for well-classified images (labels of the original and distorted images are the same) and poorly classified images (labels of the original and distorted images do not match). In addition, a more detailed comparison of the performance of explanation methods was done for the three distortions of the images. 



\subsection{Methodology}
Explanation methods' performances were analyzed on well-classified images (labels of the original and distorted images are the same) and poorly classified images (labels of the original and distorted images do not match), along with a more detailed comparison of the performance of explanation methods was done for the three distortions of the images. 

Following the result of the Kruskal-Wallis H test and Mann-Whitney U test, if the result suggests differences between the MOS of the images of the explanation methods rounded to the 4th decimal digits, the explanation methods were compared in 2 ways.
\begin{enumerate}
    \item MOS Comparison: This approach compared the MOS of the explanation methods per image, counting how many times each explanation method had a higher MOS for each image. 
    \item Mean MOS Analysis: This approach compared the mean MOS values across explanation methods. This can be seen in Tab.~\ref{tab:SA-overall}
\end{enumerate}

The result of the Kruskal-Wallis H test is shown in Tab.~\ref{tab:Kruskal-result} while the result of the Mann-Whitney U test is shown in Tab.~\ref{tab:Mann-Whitney}

\begin{table}[ht!]
    \centering
    \begin{tabular}{|c|c|c|c|c|}        
        \hline
        \rowcolor[HTML]{C0C0C0}
         \multicolumn{1}{|l|}{\backslashbox{Classification}{Distortion}}  & All             & \begin{tabular}[c]{@{}c@{}}Additive Gaussian\\ Noise\end{tabular} & \begin{tabular}[c]{@{}c@{}}Gaussian \\ Blur\end{tabular} & \begin{tabular}[c]{@{}c@{}}Uniform \\ Brightness\end{tabular} \\ \hline
Poorly                                          & \textbf{0.0012} & \textbf{0.0125}                                                   & \textbf{0.0004}                                          & 0.4111                                                        \\ \hline
Well                                            & \textbf{0.0006} & \textbf{0.0148}                                                   & 0.2899                                                   & \textbf{0.0412}                                               \\ \hline
\end{tabular}
    \caption{Table showing the p-value of the Kruskal-Wallis H test. The bold p-value indicates that there exists a statistically significant difference between the explanation methods}
    \label{tab:Kruskal-result}
\end{table}

\begin{table}[ht!]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}
    \hline
    \rowcolor[HTML]{C0C0C0}
Classification                                                                & \begin{tabular}[c]{@{}c@{}}Explanation \\ Methods\end{tabular}  & All             & \begin{tabular}[c]{@{}c@{}}Additive Gaussian \\ Noise\end{tabular} & \begin{tabular}[c]{@{}c@{}}Gaussian \\ Blur\end{tabular} & \begin{tabular}[c]{@{}c@{}}Uniform \\ Brightness\end{tabular} \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Poorly \\ Classified\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Grad-CAM \\ VS \\ MLFEM\end{tabular} & \textbf{0.0007} & 0.1677                                                             & \textbf{0.0003}                                          & N/A                                                           \\ \cline{2-6} 
                                                                              & \begin{tabular}[c]{@{}c@{}}Grad-CAM \\ VS \\ FEM\end{tabular}   & \textbf{0.0041} & \textbf{0.0042}                                                    & \textbf{0.0476}                                          & N/A                                                           \\ \cline{2-6} 
                                                                              & \begin{tabular}[c]{@{}c@{}}MLFEM \\ VS \\ FEM\end{tabular}      & 0.4954          & 0.0837                                                             & \textbf{0.0160}                                          & N/A                                                           \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Well \\ Classified\end{tabular}}   & \begin{tabular}[c]{@{}c@{}}Grad-CAM \\ VS \\ MLFEM\end{tabular} & \textbf{0.0008} & \textbf{0.0068}                                                    & N/A                                                      & \textbf{0.0340}                                               \\ \cline{2-6} 
                                                                              & \begin{tabular}[c]{@{}c@{}}Grad-CAM \\ VS \\ FEM\end{tabular}   & 0.9174          & 0.4664                                                             & N/A                                                      & 0.8683                                                        \\ \cline{2-6} 
                                                                              & \begin{tabular}[c]{@{}c@{}}MLFEM \\ VS \\ FEM\end{tabular}      & \textbf{0.0009} & \textbf{0.0294}                                                    & N/A                                                      & \textbf{0.0255}                                               \\ \hline
\end{tabular}
 \caption{Table showing the p-value of the Mann-Whitney U test. The bold p-value indicates that there exists a statistically significant difference between the explanation methods. If the Kruskal-Wallis H test suggested no significant difference between the explanation methods, the post-hoc Mann-Whitney U test was not conducted hence the ``N/A''}
    \label{tab:Mann-Whitney}
\end{table}

\begin{figure}[ht!]
     \centering
     \begin{subfigure}[b]{0.90\linewidth}
         \centering
         \includegraphics[width=\linewidth]{images/SA/MOS_analysis/Poorly Classifed.png}
         \caption{Poorly classified. The average MOS values of each explanation method can be seen in the first row (``Combined Distortion + Poor''). The average standard deviation for Grad-CAM, shown in blue, is 1.1985. For MLFEM, shown in orange, it is 1.1510, and for FEM, shown in green, it is 1.1339.}
         \label{fig:MOSALL-poor}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.90\linewidth}
         \centering
         \includegraphics[width=\linewidth]{images/SA/MOS_analysis/Correctly Classified.png}
         \caption{Well classified. The average MOS values of each explanation method can be seen in the second row (``Combined Distortion + Well''). The average standard deviation for Grad-CAM, shown in blue, is 0.8976. For MLFEM, shown in orange, it is 0.8889, and for FEM, shown in green, it is 0.8871.}
         \label{fig:MOSALL-well}
     \end{subfigure}
 \caption{MOS and the standard deviation of poorly classified and well-classified images. The images can be seen on the X-axis and MOS is shown on the Y-axis. It is interesting to note that mean MOS and mean standard deviations are globally lower for poorly classified images. This can suggest disagreements of rating among the participants.}
    \label{fig:MOSALL}
\end{figure}

% \begin{figure}[ht!]
%     \centering
%      \begin{subfigure}[b]{0.90\linewidth}
%          \centering
%         \includegraphics[width=\linewidth]{images/SA/MOS_analysis/noise_Poorly Classifed.png}
%         \caption{Poorly Classified Images with Additive Gaussian Noise}
%         \label{fig:MOSAGN-poor}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.90\linewidth}
%          \centering
%         \includegraphics[width=\linewidth]{images/SA/MOS_analysis/noise_Correctly Classified.png}
%         \caption{Well Classified Images with Additive Gaussian Noise}
%         \label{fig:MOSAGN-well}
%     \end{subfigure}
%     \caption{MOS and the standard deviation of images with additive Gaussian noise distortion. The images can be seen on the X-axis and MOS is shown on the Y-axis. Grad-CAM is shown in blue, MLFEM is shown in orange, FEM is shown in green.}
%     \label{fig:MOSAGN}
% \end{figure}

% \begin{figure}[ht!]
%     \centering
%      \begin{subfigure}[b]{0.90\linewidth}
%         \includegraphics[width=\linewidth]{images/SA/MOS_analysis/blur_Poorly Classifed.png}
%         \caption{Poorly Classified Images with Gaussian Blur Distortion}
%         \label{fig:MOSGB-poor}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.90\linewidth}
%          \centering
%         \includegraphics[width=\linewidth]{images/SA/MOS_analysis/blur_Correctly Classified.png}
%         \caption{Well Classified Images with Gaussian Blur Distortion}
%         \label{fig:MOSGB-well}
%     \end{subfigure}
%     \caption{MOS and the standard deviation of images with Gaussian blur distortion. The images can be seen on the X-axis and MOS is shown on the Y-axis. Grad-CAM is shown in blue, MLFEM is shown in orange, FEM is shown in green.}
%     \label{fig:MOSGB}
% \end{figure}

% \begin{figure}[ht!]
%     \centering
%      \begin{subfigure}[b]{0.90\linewidth}
%         \includegraphics[width=\linewidth]{images/SA/MOS_analysis/brightness_Poorly Classifed.png}
%         \caption{Poorly Classified Images with Uniform Brightness}
%         \label{fig:MOSUB-poor}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.90\linewidth}
%         \includegraphics[width=\linewidth]{images/SA/MOS_analysis/brightness_Correctly Classified.png}
%         \caption{Well Classified Images with Uniform Brightness}
%         \label{fig:MOSUB-well}
%     \end{subfigure}
%     \caption{MOS and the standard deviation of images with uniform brightness distortion. The images can be seen on the X-axis and MOS is shown on the Y-axis. Grad-CAM is shown in blue, MLFEM is shown in orange, FEM is shown in green.}
%     \label{fig:MOSUB}
% \end{figure}

\subsection{Results for Analysis of the Performance of Explanation Methods with MOS metric} \label{ssec: PerfAnalysis}

\subsubsection{Combined Distortions}
The Kruskal-Wallis H-test indicated significant differences in MOS ratings between explanation methods for poorly classified (p = 0.0012) and well-classified images (p = 0.0008). The MOS of images for explanation methods with standard deviations are presented in Fig.~\ref{fig:MOSALL}

The post-hoc Mann-Whitney U test indicated significant differences in MOS between Grad-CAM and MLFEM (p = 0.0007) and between Grad-CAM and FEM (p = 0.0041) for poorly classified images. Grad-CAM achieved a statistically higher mean MOS ($2.0940\pm0.3685$) compared to MLFEM ($1.9284\pm0.2635$). Specifically, in pairwise comparisons, Grad-CAM outperformed MLFEM on 67 out of 117 observations, while MLFEM outperformed Grad-CAM on 41 observations, with 9 ties. The mean MOS of FEM was calculated to be $1.9611\pm0.2627$ and was outperformed on 74 out of 117 images with 6 ties.

For well-classified images, the post-hoc test revealed significant differences between MLFEM and both Grad-CAM (p = 0.0008) and FEM (p = 0.0009). MLFEM obtained a statistically higher mean MOS ($3.2423\pm0.9088$) compared to Grad-CAM ($2.9190\pm0.9368$) and FEM ($2.9360\pm0.9171$). In pairwise comparisons, MLFEM outperformed Grad-CAM on 116 of 183 observations, with Grad-CAM outperforming MLFEM on 63 observations, with 4 ties. When comparing MLFEM to FEM, MLFEM performed better on 112 observations, worse on 65 observations, and there were 6 ties.


\subsubsection{Additive Gaussian Noise}
The Kruskal-Wallis H-test indicated significant differences in MOS ratings between explanation methods for poorly classified (p = 0.0125) and well-classified images (p = 0.0006) with additive Gaussian noise distortion. 
% The MOS of images for explanation methods with standard deviations are presented in Fig.~\ref{fig:MOSAGN}

The post-hoc Mann-Whitney U test indicated significant differences in MOS between Grad-CAM and FEM for poorly classified images (p = 0.0042). Grad-CAM achieved a statistically higher mean MOS ($2.1304\pm0.4061$) compared to FEM ($1.9108\pm0.2452$). Specifically, in pairwise comparisons, Grad-CAM outperformed FEM on 35 out of 46 observations, while FEM outperformed Grad-CAM on 11 observations, with 0 ties. The mean MOS of MLFEM was calculated to be $1.9910\pm0.2665$ (Grad-CAM outperformed MLFEM on 23 out of 46 images with 6 ties). 

For well-classified images, the post-hoc test revealed significant differences between MLFEM and both Grad-CAM (p = 0.0068) and FEM (p = 0.0009). MLFEM obtained a statistically higher mean MOS ($3.2471\pm0.8902$) compared to Grad-CAM ($2.7688\pm0.8902$) and FEM ($2.8870\pm0.8670$). In pairwise comparisons, MLFEM outperformed Grad-CAM on 35 of 54 observations, with Grad-CAM outperforming MLFEM on 17 observations, with 2 ties. When comparing MLFEM to FEM, MLFEM performed better on 34 observations, worse on 18 observations, and there were 2 ties.


\subsubsection{Gaussian Blur}
The Kruskal-Wallis H-test revealed a statistically significant difference in the MOS ratings assigned to explanations of poorly classified images with Gaussian blur distortion (p = 0.0004). Subsequent post-hoc pairwise Mann-Whitney U tests confirmed significant differences between all method pairs, the p-value can be seen in ~\ref{tab:Mann-Whitney}. 
% The MOS of images for explanation methods with standard deviations are presented in Fig.~\ref{fig:MOSGB}

For poorly classified images, Grad-CAM achieved the highest mean MOS ($2.2714\pm0.3689$) followed by FEM ($2.0510\pm0.2490$) and MLFEM ($1.8681\pm0.2490$). In pairwise comparisons, Grad-CAM outperformed both MLFEM (on 18 observations) and FEM (on 16 observations and 1 tie), with some instances where MLFEM (5 times) and FEM (6 times) achieved higher MOS than Grad-CAM. In addition, FEM outperformed MLFEM on 18 images out of 23 images with the same MOS on 2 images. 

The Kruskal-Wallis H-test for well-classified images with Gaussian blur distortion did not yield a statistically significant difference (p = 0.2899). This suggests that user perception of the explanation methods is not statistically different for this category.


\subsubsection{Uniform Brightness}
The Kruskal-Wallis H-test did not detect a statistically significant difference in the MOS ratings assigned to explanations of poorly classified images with uniform brightness distortion (p = 0.4111). This suggests that users perceived the explanation methods (Grad-CAM, MLFEM, and FEM) similarly for this distortion type.
% The MOS of images for explanation methods with standard deviations are presented in Fig.~\ref{fig:MOSUB}

In contrast, the Kruskal-Wallis H-test revealed a statistically significant difference in the MOS ratings for well-classified images with uniform brightness distortion (p = 0.0412). Subsequent post-hoc Mann-Whitney U tests identified significant differences between specific method pairs. Out of the 52 images, MLFEM outperformed Grad-CAM and FEM on 32 observations with 1 tie. In addition, MLFEM has the highest mean MOS ($3.3508\pm0.8353$) followed by Grad-CAM ($2.9775\pm0.9151$) and then FEM ($2.9629\pm0.8890$). 



% \subsection{Results and Discussion}

% In summary, the statistical analysis revealed significant differences in user perception of the image explanation methods (Grad-CAM \cite{DBLP:journals/corr/SelvarajuDVCPB16}, MLFEM \cite{bourroux:hal-03689004}, and FEM \cite{ahmedasiffuad:hal-02963298}) for well-classified and poorly classified images for various image distortions. These findings were based on Mean Opinion Score (MOS) as the primary user experience metric. 

% Overall, looking at Tab.~\ref{tab:SA-overall}, Grad-CAM \cite{DBLP:journals/corr/SelvarajuDVCPB16} consistently performed well for poorly classified images across the distortion types (noise, blur).
% This suggests it might be more effective in explaining image features when the model's classification is incorrect. MLFEM \cite{bourroux:hal-03689004} excelled at explaining well-classified images, particularly for distortions like additive noise and uniform brightness. This might indicate its ability to better highlight relevant image regions for correctly classified cases.
% FEM \cite{ahmedasiffuad:hal-02963298} is competitive and ties with other methods in conditions where multiple methods perform equally well, particularly on well-classified images with Gaussian blur and poorly classified images with uniform brightness. 

% For images with additive Gaussian noise, Grad-CAM \cite{DBLP:journals/corr/SelvarajuDVCPB16} outperformed FEM \cite{ahmedasiffuad:hal-02963298} for poorly classified images, while MLFEM \cite{bourroux:hal-03689004} outperformed both Grad-CAM \cite{DBLP:journals/corr/SelvarajuDVCPB16} and FEM \cite{ahmedasiffuad:hal-02963298} for well-classified images. Gaussian blur distortion resulted in significant differences between all method pairs, with Grad-CAM \cite{DBLP:journals/corr/SelvarajuDVCPB16} achieving the highest MOS overall. Uniform brightness showed no significant difference for poorly classified images, but for well-classified images, MLFEM \cite{bourroux:hal-03689004} outperformed both Grad-CAM \cite{DBLP:journals/corr/SelvarajuDVCPB16} and FEM \cite{ahmedasiffuad:hal-02963298}. These results provide valuable insights into the effectiveness of each explanation method under different image degradation conditions.



\begin{table}[ht!]
    \centering
    \begin{tabular}{|c|c|c|c|}
        \hline
        \rowcolor[HTML]{C0C0C0}
        \backslashbox{{\begin{tabular}[c]{@{}c@{}}Distortion\\ +\\ Classification\end{tabular}}}{\begin{tabular}[c]{@{}c@{}}Explanation \\ Methods\end{tabular}} & Grad-CAM & MLFEM & FEM \\\hline 
        Combined Distortion + Poor     & $\mathbf{2.0940\pm0.3685}$ & $1.9284\pm0.2635$ & $1.9611\pm0.2627$ \\ \hline
        Combined Distortion + Well     & $2.9190\pm0.9368$ & $\mathbf{3.2423\pm0.9088}$ & $2.9360\pm0.9171$ \\ \hline
        Additive Gaussian Noise + Poor & $\mathbf{2.1304\pm0.4061}$ & $1.9910\pm0.2665$ & $1.9108\pm0.2452$ \\ \hline
        Additive Gaussian Noise + Well & $2.7688\pm0.8902$ & $\mathbf{3.2471\pm0.8902}$ & $2.8870\pm0.8670$ \\ \hline
        Gaussian Blur + Poor           & $\mathbf{2.2714\pm0.3689}$ & $1.8681\pm0.2490$ & $2.0510\pm0.2490$ \\ \hline
        Gaussian Blur + Well           & $2.9848\pm0.9706$ & $3.1657\pm0.9367$ & $2.9521\pm0.9672$ \\ \hline
        Uniform Brightness + Poor      & $1.9741\pm0.2775$ & $1.8973\pm0.2551$ & $1.9662\pm0.2834$ \\ \hline
        Uniform Brightness + Well      & $2.9775\pm0.9151$ & $\mathbf{3.3508\pm0.8353}$ & $2.9629\pm0.8890$ \\ \hline
    \end{tabular}
    \caption{Table summarizing the best-performing explanation method for each distortion type and classification category. The bold value indicates the best-performing explanation method based on the mean of MOS. A tie is denoted when there are no bold values.}
    \label{tab:SA-overall}
\end{table}



\subsection{Correlation between MOS and Already Defined Metrics} \label{correlation}
% The validity of using MOS as a metric to evaluate explanation methods has been pursued by checking the correlation between MOS and already defined metrics, both automatic and semi-automatic which use Gaze Fixation Density Maps (GFDMs). We have calculated the correlation between MOS and 4 metrics, Deletion Area Under the Curve (DAUC) \cite{petsiuk2018rise}, Insertion Area Under the Curve (IAUC) \cite{DBLP:journals/corr/abs-2201-13291}


% , and the two semi-automatic metrics mentioned in Sec.~\ref{sec:XAI-metrics}.

% DAUC evaluates explanation maps by progressively masking image regions based on their importance (highest score pixels masked first). It calculates the area under the curve of the image's classification score as the masked proportion increases. A lower DAUC score indicates a better explanation because masking supposedly important regions should significantly reduce the initial score. IAUC works similarly, but in the opposite direction: it measures how revealing important areas increases the score. Pearson Correlation Coefficient (PCC) and Similarity (SIM) have been covered in Sec.~\ref{ssec:PCC} and ~\ref{ssec:SIM}. 




The validity of using MOS as a metric to evaluate explanation methods has been pursued by checking the correlation between MOS and already-defined metrics 

% , both automatic and semi-automatic which use Gaze Fixation Density Maps (GFDMs). We have calculated the correlation between MOS and 4 metrics, Deletion Area Under the Curve (DAUC) \cite{petsiuk2018rise}, Insertion Area Under the Curve (IAUC) \cite{DBLP:journals/corr/abs-2201-13291}




Looking at Tab.~\ref{tab:cor-overall}, MOS and the metrics DAUC, IAUC, PCC, and SIM for different explanation methods (All, Grad-CAM, MLFEM, and FEM) reveals distinct patterns. The ``All'' combination of methods shows moderate correlations with DAUC (0.3947) and IAUC (0.6369), but low correlations with PCC (0.1080) and SIM (0.0692). Grad-CAM follows a similar trend with moderate correlations to DAUC (0.3455) and IAUC (0.5770), and low correlations with PCC (0.1070) and SIM (0.0838). MLFEM stands out with the highest correlations to DAUC (0.4535) and IAUC (0.7033), suggesting its stronger alignment with these metrics, though it also exhibits low correlations with PCC (0.1061) and SIM (0.0755). FEM, while showing moderate correlations with DAUC (0.4009) and IAUC (0.6249), has the lowest correlation with PCC (0.0234) and a negative correlation with SIM (-0.0658), indicating a potential inverse relationship. Overall, MLFEM proves to be the most robust method in relation to DAUC and IAUC, while all methods demonstrate consistently low correlations with PCC and SIM.

\begin{table}[ht!]
\centering
\begin{tabular}{|l|l|l|l|l|}
\hline
\rowcolor[HTML]{C0C0C0}
         & DAUC   & IAUC   & PCC    & SIM     \\ \hline
All      & 0.3947 & 0.6369 & 0.1080 & 0.0692  \\ \hline
Grad-CAM & 0.3455 & 0.5770 & \textbf{0.1070} & \textbf{0.0838}  \\ \hline
MLFEM    & \textbf{0.4535} & \textbf{0.7033} & 0.1061 & 0.0755  \\ \hline
FEM      & 0.4009 & 0.6249 & 0.0234 & -0.0658 \\ \hline
\end{tabular}
\caption{Table showing Pearson coefficient correlation between MOS of explanation methods and already defined metrics. all is for all the explanation methods combined.}
\label{tab:cor-overall}
\end{table}

% \clearpage % You need \clearpage at the end of every chapter to force images included in this chapter to be rendered somewhere within it











==> contents/6-results-SA.tex <==
\section{Results} \label{result-SA}
% The Code of Studies and Exams recommends the following content for this chapter: "Evaluation, critical analysis of the implemented technical solutions, possibilities for further development."
% However, you are free to structure the content of your thesis as you want
This section presents the results of the statistical analysis conducted to evaluate the performance of the explanation methods (Grad-CAM \cite{DBLP:journals/corr/SelvarajuDVCPB16}, MLFEM \cite{bourroux:hal-03689004}, and FEM \cite{ahmedasiffuad:hal-02963298}) described in Section \ref{SA}. The analysis focused on Mean Opinion Score (MOS) as the primary user experience metric. We investigated potential differences in user perception of the explanation methods for two categories of distorted images: well-classified (labels of original and distorted images match) and poorly-classified (labels differ). The analysis employed the Kruskal-Wallis H test \cite{doi:10.1080/01621459.1952.10483441} to identify statistically significant differences in MOS ratings across explanation methods for each distortion type. In cases where significant differences were found, post-hoc Mann-Whitney U tests \cite{10.1214/aoms/1177730491} were conducted for pairwise comparisons between methods. The results are presented for three common image distortions: additive Gaussian noise, Gaussian blur, and uniform brightness (Section \ref{sec:Methods-Degraded-Image-Set}).

\subsection{Results for Analysis of the Performance of Explanation Methods with MOS metric} \label{ssec: PerfAnalysis}
The performance of explanation methods was analyzed for each type of degradation of well-classified images (labels of the original and distorted images are the same) and poorly classified images (labels of the original and distorted images do not match). 

Following the result of the Kruskal-Wallis H test and Mann-Whitney U test, if the result suggests differences between the MOS of the images of the explanation methods rounded to the 4th decimal digits, the explanation methods were compared in 2 ways.
\begin{enumerate}
    \item MOS Comparison: This approach directly compared the MOS values of the images associated with each explanation method for the specific degradation type. The goal was to identify which method yielded higher average user ratings.
    \item Mean MOS Analysis: This approach compared the mean MOS values across explanation methods for the specific degradation type. This provided a more comprehensive understanding of overall user perception differences.
\end{enumerate}

The performance of explanation methods was evaluated for two categories of distorted images:
\begin{itemize}
    \item Well-classified: Images where the labels of the original and distorted versions are identical.
    \item Poorly classified: Images where the labels of the original and distorted versions differ.
\end{itemize}
    
The MOS of images for explanation methods with standard deviations are presented in Fig.~\ref{fig:MOSAGN} for additive Gaussian noise, in Fig.~\ref{fig:MOSGB} for Gaussian blur, and in Fig.~\ref{fig:MOSUB} for uniform brightness.

\subsubsection{Additive Gaussian Noise}
The Kruskal-Wallis H-test indicated significant differences in MOS ratings between explanation methods for both poorly classified (p = 0.0167) and well-classified images (p = 0.0135) with additive Gaussian noise distortion (Tab.~\ref{tab:KWHT-AGN}). Subsequent Mann-Whitney U tests (Tab.~\ref{tab:MWUT-AGN}) revealed that Grad-CAM outperformed FEM for poorly classified images (p = 0.0065). 

The post-hoc Mann-Whitney U test indicated significant differences in MOS between Grad-CAM and FEM for poorly classified images. Grad-CAM achieved a statistically higher mean MOS ($2.1592\pm0.4232$) compared to FEM ($1.9286\pm0.2525$). Specifically, in pairwise comparisons, Grad-CAM outperformed FEM on 34 out of 46 observations, while FEM outperformed Grad-CAM on 11 observations, with 1 tie. The mean MOS of MLFEM was calculated to be $2.0093\pm0.2741$. 

For well-classified images, the post-hoc test revealed significant differences between MLFEM and both Grad-CAM and FEM. MLFEM obtained a statistically higher mean MOS ($3.2407\pm0.9337$) compared to Grad-CAM ($2.7493\pm0.8944$) and FEM ($2.8796\pm0.8804$). It's important to note that there were no ties in the MLFEM vs Grad-CAM comparison. In pairwise comparisons, MLFEM outperformed Grad-CAM on 38 out of 54 observations, with Grad-CAM outperforming MLFEM on 16 observations. When comparing MLFEM to FEM, MLFEM performed better on 35 observations, worse on 18 observations, and there was 1 tie.

\begin{table}[!ht]
    \centering
    \begin{tabular}{|l|l|}
        \hline
        \rowcolor[HTML]{C0C0C0} 
        Classification &P-Value \\ \hline
        \textbf{Poor}  &\textbf{0.0167}  \\ \hline
        \textbf{Well}  &\textbf{0.0135}  \\ \hline    
    \end{tabular}
    \caption{Kruskal-Wallis H Test of Additive Gaussian Noise Distortion}
    \label{tab:KWHT-AGN}
\end{table} 
\begin{table}[!ht]
    \begin{subtable}[b]{0.45\linewidth}   
        \centering
        \begin{tabular}{|l|l|l|l|l|l|}
            \hline
            \rowcolor[HTML]{C0C0C0}
            Explanation Methods &P-Value  \\ \hline
            Grad-CAM VS MLFEM   &0.1313    \\ \hline
            \textbf{Grad-CAM VS FEM}     &\textbf{0.0065}    \\ \hline
            MLFEM VS FEM        &0.1088    \\ \hline
        \end{tabular}
        \caption{Poorly Classified Images}
    \end{subtable}
    \begin{subtable}[b]{0.45\linewidth}   
        \centering
        \begin{tabular}{|l|l|l|l|l|l|}
            \hline
            \rowcolor[HTML]{C0C0C0}
            Explanation Methods &P-Value  \\ \hline
            \textbf{Grad-CAM VS MLFEM}   &\textbf{0.0055}    \\ \hline
            Grad-CAM VS FEM     &0.4405    \\ \hline
            \textbf{MLFEM VS FEM}        &\textbf{0.0330}    \\ \hline
        \end{tabular}
        \caption{Well Classified Images}
    \end{subtable}
    \caption{Mann-Whitney U Test Result of Additive Gaussian Noise Distortion}
        \label{tab:MWUT-AGN}
\end{table} 
\begin{figure}[ht!]
    \begin{minipage}{0.90\linewidth}
        \includegraphics[width=\linewidth]{images/SA/MOS_analysis/noise_Poorly Classifed.png}
        \caption{Poorly Classified}
        % \label{}
    \end{minipage}
    \\
    % \hfill
    \begin{minipage}{0.90\linewidth}
        \includegraphics[width=\linewidth]{images/SA/MOS_analysis/noise_Correctly Classified.png}
        \caption{Well Classified}
        % \label{}
    \end{minipage}
    \caption{MOS and the Standard Deviation of Images with Additive Gaussian Noise Distortion. The images can be seen on the X-axis along with MOS shown on the Y-axis.}
    \label{fig:MOSAGN}
\end{figure}

\subsubsection{Gaussian Blur}
Looking at Fig.~\ref{fig:MOSGB}, the Kruskal-Wallis H-test revealed a statistically significant difference in the MOS ratings assigned to explanations of images with Gaussian blur distortion (p = 0.0006; Tab.~\ref{tab:KWHT-GB}). Subsequent post-hoc pairwise Mann-Whitney U tests (Tab.~\ref{tab:MWUT-GB}) confirmed significant differences between all method pairs.

Grad-CAM achieved the highest mean MOS ($2.2935\pm0.3790$) followed by FEM ($2.0637\pm0.2383$) and MLFEM ($1.8913\pm0.2649$). In pairwise comparisons, Grad-CAM outperformed both MLFEM (on 18 observations) and FEM (on 16 observations), with some instances where MLFEM (5 times) and FEM (6 times) achieved higher MOS than Grad-CAM. In addition, FEM outperformed MLFEM on 15 images out of 23 images with the same MOS on 3 images. 

The Kruskal-Wallis H-test for well-classified images with Gaussian blur distortion did not yield a statistically significant difference (p = 0.2810). This suggests that user perception of the explanation methods is not statistically different for this category.

\begin{table}[!ht]
    \centering
    \begin{tabular}{|l|l|}
        \hline
        \rowcolor[HTML]{C0C0C0} 
        Classification &P-Value \\ \hline
        \textbf{Poor}  &\textbf{0.0006}  \\ \hline
        Well  &0.2810  \\ \hline    
    \end{tabular}
    \caption{Kruskal-Wallis H Test of Gaussian Blur Distortion}
    \label{tab:KWHT-GB}
\end{table} 
\begin{table}[!ht]
    \centering
    \begin{tabular}{|l|l|l|l|l|l|}
        \hline
        \rowcolor[HTML]{C0C0C0}
        Explanation Methods &P-Value  \\ \hline
        \textbf{Grad-CAM VS MLFEM}   &\textbf{0.0003}    \\ \hline
        \textbf{Grad-CAM VS FEM}     &\textbf{0.0375}    \\ \hline
        \textbf{MLFEM VS FEM}        &\textbf{0.3264}    \\ \hline
    \end{tabular}   
    \caption{Mann-Whitney U Test Result of Poorly Classified Images with Gaussian Blur Distortion}
        \label{tab:MWUT-GB}
\end{table} 
\begin{figure}[ht!]
    \begin{minipage}{0.90\linewidth}
        \includegraphics[width=\linewidth]{images/SA/MOS_analysis/blur_Poorly Classifed.png}
        \caption{Poorly Classified}
        % \label{}
    \end{minipage}
    \\
    % \hfill
    \begin{minipage}{0.90\linewidth}
        \includegraphics[width=\linewidth]{images/SA/MOS_analysis/blur_Correctly Classified.png}
        \caption{Well Classified}
        % \label{}
    \end{minipage}
    \caption{MOS and the Standard Deviation of Images with Gaussian Blur Distortion. The images can be seen on the X-axis along with MOS shown on the Y-axis.}
    \label{fig:MOSGB}
\end{figure}

\subsubsection{Uniform Brightness Distortion}
The Kruskal-Wallis H-test did not detect a statistically significant difference in the MOS ratings assigned to explanations of images with uniform brightness distortion (p = 0.5240; Tab.~\ref{tab:KWHT-UB}). This suggests that users perceived the explanation methods (Grad-CAM, MLFEM, and FEM) similarly for this distortion type.

In contrast, the Kruskal-Wallis H-test revealed a statistically significant difference in the MOS ratings for well-classified images with uniform brightness distortion (p = 0.0486; Tab,~\ref{tab:KWHT-UB}). Subsequent post-hoc Mann-Whitney U tests (Tab.~\ref{tab:MWUT-UB}) identified significant differences between specific method pairs. MLFEM outperformed Grad-CAM (on 33 observations) and FEM (on 33 observations), with some instances where Grad-CAM (18 times) and FEM (18 times) achieved higher MOS than MLFEM (details in the provided dictionary). In addition, MLFEM has the highest mean MOS ($3.3764\pm0.8506$) followed by FEM ($2.9945\pm0.9131$) and Grad-CAM ($2.9931\pm0.9421$). The MOS and the standard deviation of the explanation methods for the images can be seen in Fig.~\ref{fig:MOSAGN}.

\begin{table}[!ht]
    \centering
    \begin{tabular}{|l|l|}
        \hline
        \rowcolor[HTML]{C0C0C0} 
        Classification &P-Value \\ \hline
        Poor  &0.5294  \\ \hline
        \textbf{Well}  &\textbf{0.0486}  \\ \hline    
    \end{tabular}
    \caption{Kruskal-Wallis H Test of Uniform Brightness Distortion}
    \label{tab:KWHT-UB}
\end{table} 
\begin{table}[!ht]
    \centering
    \begin{tabular}{|l|l|l|l|l|l|}
        \hline
        \rowcolor[HTML]{C0C0C0}
        Explanation Methods &P-Value   \\ \hline
        \textbf{Grad-CAM VS MLFEM}   &\textbf{0.0380}    \\ \hline
        Grad-CAM VS FEM     &0.9896    \\ \hline
        \textbf{MLFEM VS FEM}        &\textbf{0.0299}    \\ \hline
    \end{tabular}   
    \caption{Mann-Whitney U Test Result of Well Classified Images with Uniform Brightness Distortion}
        \label{tab:MWUT-UB}
\end{table} 
\clearpage
\begin{figure}[ht!]
    \begin{minipage}{0.90\linewidth}
        \includegraphics[width=\linewidth]{images/SA/MOS_analysis/brightness_Poorly Classifed.png}
        \caption{Poorly Classified}
        % \label{}
    \end{minipage}
    \\
    % \hfill
    \begin{minipage}{0.90\linewidth}
        \includegraphics[width=\linewidth]{images/SA/MOS_analysis/brightness_Correctly Classified.png}
        \caption{Well Classified}
        % \label{}
    \end{minipage}
    \caption{MOS and the Standard Deviation of Images with Uniform Brightness Distortion. The images can be seen on the X-axis along with MOS shown on the Y-axis.}
    \label{fig:MOSUB}
\end{figure}

\subsection{Discussion}

In summary, the statistical analysis revealed significant differences in user perception of the image explanation methods (Grad-CAM \cite{DBLP:journals/corr/SelvarajuDVCPB16}, MLFEM \cite{bourroux:hal-03689004}, and FEM \cite{ahmedasiffuad:hal-02963298}) for various image distortions. These findings were based on Mean Opinion Score (MOS) as the primary user experience metric. The analysis focused on two image categories: well-classified (original and distorted labels match) and poorly-classified (labels differ).

For images with additive Gaussian noise, Grad-CAM \cite{DBLP:journals/corr/SelvarajuDVCPB16} outperformed FEM \cite{ahmedasiffuad:hal-02963298} for poorly classified images, while MLFEM \cite{bourroux:hal-03689004} outperformed both Grad-CAM \cite{DBLP:journals/corr/SelvarajuDVCPB16} and FEM \cite{ahmedasiffuad:hal-02963298} for well-classified images. Gaussian blur distortion resulted in significant differences between all method pairs, with Grad-CAM \cite{DBLP:journals/corr/SelvarajuDVCPB16} achieving the highest MOS overall. Uniform brightness showed no significant difference for poorly classified images, but for well-classified images, MLFEM \cite{bourroux:hal-03689004} outperformed both Grad-CAM \cite{DBLP:journals/corr/SelvarajuDVCPB16} and FEM \cite{ahmedasiffuad:hal-02963298}. These results provide valuable insights into the effectiveness of each explanation method under different image degradation conditions.

Overall, looking at Tab.~\ref{tab:SA-overall}, Grad-CAM \cite{DBLP:journals/corr/SelvarajuDVCPB16} consistently performed well for poorly classified images across the distortion types (noise, blur).
This suggests it might be more effective in explaining image features when the model's classification is incorrect. MLFEM \cite{bourroux:hal-03689004} excelled at explaining well-classified images, particularly for distortions like additive noise and uniform brightness. This might indicate its ability to better highlight relevant image regions for correctly classified cases.
FEM \cite{ahmedasiffuad:hal-02963298} is competitive and ties with other methods in conditions where multiple methods perform equally well, particularly on well-classified images with Gaussian blur and poorly classified images with uniform brightness. 


\begin{table}[ht!]
    \centering
    \begin{tabular}{|l|l|l|l|}
        \hline
        \rowcolor[HTML]{C0C0C0}
        \backslashbox{Distortion+Classification}{Explanation Methods} 
         & Grad-CAM & MLFEM & FEM \\\hline
        Additive Gaussian Noise + Poor                   & *        &       &     \\ \hline
        Additive Gaussian Noise + Well                   &          & *     &     \\ \hline
        Gaussian Blur + Poor                             & *        &       &     \\ \hline
        Gaussian Blur + Well                             & *        & *     & *   \\ \hline
        Uniform Brightness + Poor                        & *        & *     & *   \\ \hline
        Uniform Brightness + Well                        &          & *     &    \\ \hline
        \end{tabular}
    \caption{Table summarizing the best-performing explanation method for each image degradation type and classification category. An asterisk (*) indicates the best-performing method based on MOS. A tie is denoted when all methods have an asterisk.
}
    \label{tab:SA-overall}
\end{table}


% \clearpage % You need \clearpage at the end of every chapter to force images included in this chapter to be rendered somewhere within it











==> contents/appendices.tex <==
\chapter{Appendix A} 
Here you can present all the materials that help the understanding of your work, but either 1) not your work, 2) not necessary to understanding, 3) simply just interesting things not directly related to your topic, or 4) your text already exceeded 120 pages, and need to make it shorter by moving parts to appendix... Also, if you have a large number of images, code, or measurement data, it is required to insert them here rather than in chapters. You can have multiple appendices (possibly separated into multiple files) as it suits the content of the supplemental material.

